A Hybrid Quasi-Newton Projected-Gradient Method with Application to Lasso and Basis-Pursuit Denoise

We propose a new algorithm for the optimization of convex functions over a polyhedral set in Rn. The algorithm extends the spectral projected-gradient method with limited-memory BFGS iterates restricted to the present face whenever possible. We prove convergence of the algorithm under suitable conditions and apply the algorithm to solve the Lasso problem, and consequently, the basis-pursuit denoise problem through the root-finding framework proposed by van den Berg and Friedlander [SIAM Journal on Scientific Computing, 31(2), 2008]. The algorithm is especially well suited to simple domains and could also be used to solve bound-constrained problems as well as problems restricted to the simplex.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        macros.tex                                  %
%                                                    %
% Current version: Michael P. Friedlander            %
%                  Dept of Computer Science          %
%                  University of British Columbia    %
%                                                    %
% 1998: Derived from Michael Saunders's macros file. %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% $Revision: 1.2 $ $Date: 2004-04-20 10:18:51-05 $
% 13 Mar 1999: Added Abract environment
% 11 May 2000: Added several theorem environments
% 08 Jun 2001: Deleted absract environment
% 09 Nov 2001: Using RequirePackage to load req'd packages
% 21 Mar 2004: Deleted lots of never-used macros.  Cleanup.
% 06 Jul 2005: Using mathbb instead of mathds.  Looks better.

%%%%%%%%%%%
%  Packages
%%%%%%%%%%%
\RequirePackage{amsmath}
\RequirePackage{amssymb}
%\RequirePackage{dsfont}

%%%%%%%%%%%%%%%%%%%
% -- AMSMATH tweak:
% Subassumptions environment similar to subequations.
%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcounter{parenttheorem}%
\newenvironment{subassumptions}{%
  \refstepcounter{theorem}%
  \protected@edef\theparenttheorem{\thetheorem}%
  \setcounter{parenttheorem}{\value{theorem}}%
  \setcounter{theorem}{0}%
  \def\thetheorem{\theparenttheorem\normalfont\alph{theorem}}%
  \ignorespaces
}{%
  \setcounter{theorem}{\value{parenttheorem}}%
  \ignorespacesafterend
}
\makeatother

%%%%%%%%%%%%%%%%%%%
% BibTeX macro.  Taken from /usr/share/texmf/doc/bibtex/base/btxdoc.tex.
%%%%%%%%%%%%%%%%%%%
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\tild{\raisebox{-0.5ex}{\~{}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Minimize, maximize, subject to
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\minim{\mathop{\hbox{minimize}}}
\def\maxim{\mathop{\hbox{maximize}}}
\def\minimize#1{\displaystyle\minim_{#1}}
\def\maximize#1{\displaystyle\maxim_{#1}}
\def\st{\mathop{\hbox{subject to}}}
\def\argmin{\mathop{\hbox{arg\,min}}}
\def\argmax{\mathop{\hbox{arg\,max}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Max/Min Problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\uncprob#1#2#3{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{9pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $
    \end{tabular*}}}
\def\problem#1#2#3#4{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\problemnb#1#2#3#4{
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probwide#1#2#3#4{\fbox
  {\begin{tabular*}{.98\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probnarrow#1#2#3#4{\fbox
  {\begin{tabular*}{0.7\paperwidth}
      {@{}l@{\extracolsep{\fill}}c@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\makeatother

\def\dps\displaystyle
\def\clink#1{\mkern2mu\overline{\mkern-2mu c\mkern2mu}\mkern-2mu\k(#1)}
\def\ul#1{\underline{#1}}
\def\Real{\mathbb{R}}
\def\Symm{\mathbb{S}}
\def\Complex{\mathbb{C}}
\def\m{\phantom-}
%\def\eval#1#2{\left.#2\right|_{\alpha=#1}}
% Matrices and vectors
%\def\tmat#1#2{(\, #1 \ \ #2 \,)}
%\def\tmatt#1#2#3{(\, #1 \ \  #2 \ \  #3\,)}
%\def\tmattt#1#2#3#4{(\, #1 \ \  #2 \ \  #3 \ \  #4\,)}
%\def\mat#1#2{(\; #1 \quad #2 \;)}
%\def\matt#1#2#3{(\; #1 \quad #2 \quad #3\;)}
%\def\mattt#1#2#3#4{(\; #1 \quad #2 \quad #3 \quad #4\;)}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\comp#1#2{[#2]_{#1}}
\def\compi#1{[#1]_i}
\def\compj#1{[#1]_j}
%\def\defd{\raisebox{-.2ex}{$\stackrel{\mathrm{def}}{=}$}}
\def\defd{\mathrel{\mathop:}=} % As per Higham's ``Accuracy & Stability...''
\def\abs#1{|#1|}
\def\norm#1{\|#1\|}
\def\onenorm#1{\|#1\|_1}
\def\twonorm#1{\|#1\|_2}
\def\infnorm#1{\norm{#1}_\infty}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 6pt depth 1.5pt
  \hskip 1pt}}
\def\cross{{\scriptscriptstyle\times}}
\def\cond{\hbox{\rm cond}}
\def\det{\mathop{\hbox{\rm det}}}
\def\diag{\operatorname{diag}}
\def\dim{\mathop{\hbox{\rm dim}}}  
\def\boundary{\mathop{\hbox{\rm bnd}}}
\def\interior{\mathop{\hbox{\rm int}}}
\def\Null{\mathop{\hbox{\rm null}}}
\def\rank{\mathop{\hbox{\rm rank}}}
\def\op{\mathop{\hbox{\rm op}}}
\def\range{\mathop{\hbox{\rm range}}}
\def\sign{\operatorname{sign}}
\def\sgn{\operatorname{sgn}}
\def\Span{\mbox{\rm span}}
\def\trace{\mathop{\hbox{\rm trace}}}
\def\drop{^{\null}}
\def\float{fl}
\def\grad#1{\nabla_{#1}}
\def\Hess#1{\nabla^2_{#1}}
\def\one{\mathbf{1}}
\def\half{{\textstyle{\frac{1}{2}}}}
\def\third{{\textstyle{\frac{1}{3}}}}
\def\fourth{{\textstyle{\frac{1}{4}}}}
\def\inv{^{-1}}
\def\invsq{^{-2}}
\def\limk{\lim_{k\to\infty}}
\def\mystrut{\vrule height10.5pt depth5.5pt width0pt}
\def\spose#1{\hbox to 0pt{#1\hss}}
\def\sub#1{^{\null}_{#1}}
\def\text #1{\hbox{\quad#1\quad}}
\def\textt#1{\hbox{\qquad#1\qquad}}
\def\invT{^{-T}\!}
\def\T{^T\!}
\def\pT{^{+T}}
\def\xint{{x_{\rm int}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Fixed-size glue, only for math mode
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pthinsp{\mskip  2   mu}    %           thin space
\def\pmedsp {\mskip  2.75mu}    %         medium space
\def\pthiksp{\mskip  3.5 mu}    %          thick space
\def\nthinsp{\mskip -2   mu}
\def\nmedsp {\mskip -2.75mu}
\def\nthiksp{\mskip -3.5 mu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Specially lowered subscripts (see \sub above)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Asubk{A\sub{\nthinsp k}}
\def\Bsubk{B\sub{\nthinsp k}}
\def\Fsubk{F\sub{\nmedsp k}}
\def\Gsubk{G\sub{\nthinsp k}}
\def\Hsubk{H\sub{\nthinsp k}}
\def\HsubB{H\sub{\nthinsp  \scriptscriptstyle{B}}}
\def\HsubS{H\sub{\nthinsp  \scriptscriptstyle{S}}}
\def\HsubBS{H\sub{\nthinsp \scriptscriptstyle{BS}}}
\def\Hz{H\sub{\nthinsp \scriptscriptstyle{Z}}}
\def\Jsubk{J\sub{\nmedsp k}}
\def\Psubk{P\sub{\nthiksp k}}
\def\Qsubk{Q\sub{\nthinsp k}}
\def\Vsubk{V\sub{\nmedsp k}}
\def\Vsubone{V\sub{\nmedsp 1}}
\def\Vsubtwo{V\sub{\nmedsp 2}}
\def\Ysubk{Y\sub{\nmedsp k}}
\def\Wsubk{W\sub{\nthiksp k}}
\def\Zsubk{Z\sub{\nthinsp k}}
\def\Zsubi{Z\sub{\nthinsp i}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Subscripts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\submax{_{\max}}
\def\submin{_{\min}}
\def\subminus{_{\scriptscriptstyle -}}
\def\subplus {_{\scriptscriptstyle +}}

\def\A{_{\scriptscriptstyle A}}
\def\B{_{\scriptscriptstyle B}}
\def\C{_{\scriptscriptstyle C}}
\def\D{_{\scriptscriptstyle D}}
\def\E{_{\scriptscriptstyle E}}
\def\F{_{\scriptscriptstyle F}}
\def\G{_{\scriptscriptstyle G}}
\def\H{_{\scriptscriptstyle H}}
\def\I{_{\scriptscriptstyle I}}
\def\J{_{\scriptscriptstyle J}}
\def\K{_{\scriptscriptstyle K}}
\def\L{_{\scriptscriptstyle L}}
\def\M{_{\scriptscriptstyle M}}
\def\N{_{\scriptscriptstyle N}}
\def\O{_{\scriptscriptstyle O}}
\def\P{_{\scriptscriptstyle P}}
\def\Q{_{\scriptscriptstyle Q}}
\def\R{_{\scriptscriptstyle R}}
\def\U{_{\scriptscriptstyle U}}
\def\V{_{\scriptscriptstyle V}}
\def\W{_{\scriptscriptstyle W}}
\def\Y{_{\scriptscriptstyle Y}}
\def\Z{_{\scriptscriptstyle Z}}
\def\k{_k}
\def\kp#1{_{k+#1}}
\def\km#1{_{k-#1}}
\def\j{_j}
\def\jp#1{_{j+#1}}
\def\jm#1{_{j-#1}}
\def\subb{\B}
\def\subc{\C}
\def\subf{\F}
\def\subh{\H}
\def\subk{\K}
\def\subm{\M}
\def\subn{\N}
\def\subp{\P}
\def\subs{_{\scriptscriptstyle S}}
\def\subt{_{\scriptscriptstyle T}}
\def\subr{\R}
\def\subz{\Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  bars, hats, tildes  (\skew4 is the default)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\alphabar{\bar \alpha}
\def\alphahat{\skew3\hat \alpha}
\def\alphatilde{\skew3\tilde \alpha}
\def\betabar{\skew{2.8}\bar\beta}
\def\betahat{\skew{2.8}\hat\beta}
\def\betatilde{\skew{2.8}\tilde\beta}
\def\deltabar{\bar\delta}
\def\deltilde{\skew5\tilde \delta}
\def\deltatilde{\deltilde}
\def\etabar{\bar\eta}
\def\gammabar{\bar\gamma}
\def\lambar{\bar\lambda}
\def\lamhat{\skew{2.8}\hat \lambda}
\def\lambdahat{\lamhat}
\def\lambdatilde{\tilde{\lambda}}
\def\lambdabar{\bar \lambda}
\def\mubar{\skew3\bar \mu}
\def\muhat{\skew3\hat \mu}
\def\mutilde{\skew3\tilde\mu}
\def\nubar{\skew3\bar\nu}
\def\nuhat{\skew3\hat\nu}
\def\nutilde{\skew3\tilde\nu}
\def\omegabar{\bar\omega}
\def\omegahat{\skew3\hat\omega}
\def\omegatilde{\tilde\omega}
\def\phibar{\bar\phi}
\def\pibar{\bar\pi}
\def\pihat{\skew1\widehat \pi}
\def\sigmaB{\mkern 3mu\overline {\mkern-3mu\sigma\mkern 1mu}\mkern-1mu}
\def\sigmab{\mkern-2mu\underline{\mkern 2mu\sigma\mkern-3mu}\mkern 3mu}
\def\sigmabar{\bar\sigma}
\def\rhobar{\bar\rho}
\def\rhohat{\widehat\rho}
\def\taubar{\bar\tau}
\def\tautilde{\tilde\tau}
\def\tauhat{\hat\tau}
\def\thetabar{\bar\theta}
\def\xibar{\skew4\bar\xi}

\def\abar{\skew3\bar a}
\def\ahat{\skew2\widehat a}
\def\atilde{\skew2\widetilde a}
\def\Abar{\skew7\bar A}
\def\Ahat{\widehat A}
\def\Atilde{\widetilde A}
\def\bbar{\skew3\bar b}
\def\bhat{\skew2\widehat b}
\def\btilde{\skew2\widetilde b}
\def\Bbar{\bar B}
\def\Bhat{\widehat B}
\def\cbar{\skew3\bar c}
\def\chat{\skew3\widehat c}
\def\ctilde{\widetilde c}
\def\Cbar{\bar C}
\def\Chat{\widehat C}
\def\Ctilde{\widetilde C}
\def\dbar{\bar d}
\def\dhat{\widehat d}
\def\dtilde{\widetilde d}
\def\Dbar{\bar D}
\def\Dhat{\widehat D}
\def\Dtilde{\widetilde D}
\def\ehat{\skew3\widehat e}
\def\ebar{\bar e}
\def\Ebar{\bar E}
\def\Ehat{\widehat E}
\def\Etilde{\widetilde E}
\def\fbar{\bar f}
\def\fhat{\widehat f}
\def\ftilde{\widetilde f}
\def\Fbar{\bar F}
\def\Fhat{\widehat F}
\def\Ftilde{\widetilde F}
\def\gbar{\skew{4.3}\bar g}
\def\ghat{\skew{3}\widehat g}
\def\gtilde{\skew{4.5}\widetilde g}
\def\Gbar{\bar G}
\def\Ghat{\widehat G}
\def\hbar{\skew{4.2}\bar h}
\def\hhat{\skew2\widehat h}
\def\htilde{\skew3\widetilde h}
\def\Hbar{\skew5\bar H}
\def\Hhat{\widehat H}
\def\Htilde{\widetilde H}
\def\Ibar{\skew5\bar I}
\def\Itilde{\widetilde I}
\def\Jbar{\skew6\bar J}
\def\Jhat{\widehat J}
\def\Jtilde{\widetilde J}
\def\kbar{\skew{4.4}\bar k}
\def\Khat{\widehat K}
\def\Kbar{\skew{4.4}\bar K}
\def\Ktilde{\widetilde K}
\def\ellbar{\bar \ell}
\def\lhat{\skew2\widehat l}
\def\lbar{\skew2\bar l}
\def\Lbar{\skew{4.3}\bar L}
\def\Lhat{\widehat L}
\def\Ltilde{\widetilde L}
\def\mbar{\skew2\bar m}
\def\mhat{\widehat m}
\def\Mbar{\skew{4.4}\bar M}
\def\Mhat{\widehat M}
\def\Mtilde{\widetilde M}
\def\Nbar{\skew{4.4}\bar N}
\def\Ntilde{\widetilde N}
\def\nbar{\skew2\bar n}
\def\pbar{\skew2\bar p}
\def\phat{\skew2\widehat p}
\def\ptilde{\skew2\widetilde p}
\def\Pbar{\skew5\bar P}
\def\Phat{\widehat P}
\def\Ptilde{\skew5\widetilde P}
\def\qbar{\bar q}
\def\qhat{\skew2\widehat q}
\def\qtilde{\widetilde q}
\def\Qbar{\bar Q}
\def\Qhat{\widehat Q}
\def\Qtilde{\widetilde Q}
\def\rbar{\skew3\bar r}
\def\rhat{\skew3\widehat r}
\def\rtilde{\skew3\widetilde r}
\def\Rbar{\skew5\bar R}
\def\Rhat{\widehat R}
\def\Rtilde{\widetilde R}
\def\sbar{\bar s}
\def\shat{\widehat s}
\def\stilde{\widetilde s}
\def\Shat{\widehat S}
\def\Sbar{\skew2\bar S}
\def\tbar{\bar t}
\def\ttilde{\widetilde t}
\def\that{\widehat t}
\def\Tbar{\bar T}
\def\That{\widehat T}
\def\Ttilde{\widetilde T}
\def\ubar{\skew3\bar u}
\def\uhat{\skew3\widehat u}
\def\utilde{\skew3\widetilde u}
\def\Ubar{\skew2\bar U}
\def\Uhat{\widehat U}
\def\Utilde{\widetilde U}
\def\vbar{\skew3\bar v}
\def\vhat{\skew3\widehat v}
\def\vtilde{\skew3\widetilde v}
\def\Vbar{\skew2\bar V}
\def\Vhat{\widehat V}
\def\Vtilde{\widetilde V}
\def\wbar{\skew3\bar w}
\def\what{\skew3\widehat w}
\def\wtilde{\skew3\widetilde w}
\def\Wbar{\skew3\bar W}
\def\What{\widehat W}
\def\Wtilde{\widetilde W}
\def\xbar{\bar{x}}
\def\xhat{\skew{2.8}\widehat x}
\def\xtilde{\skew3\widetilde x}
\def\Xhat{\widehat X}
\def\ybar{\skew3\bar y}
\def\yhat{\skew2\widehat y}
\def\ytilde{\skew3\widetilde y}
\def\Ybar{\skew2\bar Y}
\def\Yhat{\widehat Y}
\def\zbar{\skew{2.8}\bar z}
\def\zhat{\skew{2.8}\widehat z}
\def\ztilde{\skew{2.8}\widetilde z}
\def\Zbar{\skew5\bar Z}
\def\Zhat{\widehat Z}
\def\Ztilde{\widetilde Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Stars
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lamstar{\lambda^*}
\def\lamstark{\lambda^*\k}
\def\lambarstark{\lambar^*\k}
\def\pistar{\pi^*}
\def\pistark{\pi^*_k}
\def\rhostar{\rho^*}
\def\mustar{\mu^*}
\def\taustar{\tau^*}
\def\cstar{c^*}
\def\dstar{d^*}
\def\gstar{g^*}
\def\Jstar{J^*}
\def\pstar{p^*}
\def\rstar{r^*}
\def\rstark{r^*\k}
\def\vstar{v^*}
\def\vstark{v^*\k}
\def\wstar{w^*}
\def\wstark{w^*\k}
\def\xstar{x^*}
\def\xstarhatk{\hat x^*\k}
\def\xstark{x^*\k}
\def\xstarzero{x^*_0}
\def\xstarkm1{x^*\km1}
\def\ystar{y^*}
\def\ystarhatk{\hat y^*\k}
\def\ystark{y^*\k}
\def\ystarkm1{y^*\km1}
\def\zstar{z^*}
\def\zstark{z^*\k}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math italic fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mit{\mathit}
\def\Deltait{{\mit \Delta}}
\def\Gammait{{\mit \Gamma}}
\def\Lambdait{{\mit \Lambda}}
\def\Sigmait{{\mit \Sigma}}
\def\Lambarit{\skew5\bar{\mit \Lambda}}
\def\Omegait{{\mit \Omega}}
\def\Omegaitbar{\skew5\bar{\mit \Omega}}
\def\Thetait{{\mit \Theta}}
\def\Piitbar{\skew5\bar{\mit \Pi}}
\def\Piit{{\mit \Pi}}
\def\Phiit{{\mit \Phi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math calligraphy fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lscr{\ell}
\def\Ascr{\mathcal{A}}
\def\Bscr{\mathcal{B}}
\def\Cscr{\mathcal{C}}
\def\Escr{\mathcal{E}}
\def\Fscr{\mathcal{F}}
\def\Dscr{\mathcal{D}}
\def\Iscr{\mathcal{I}}
\def\Jscr{\mathcal{J}}
\def\Kscr{\mathcal{K}}
\def\Lscr{\mathcal{L}}
\def\Mscr{\mathcal{M}}
\def\Nscr{\mathcal{N}}
\def\Oscr{\mathcal{O}}
\def\Pscr{\mathcal{P}}
\def\Qscr{\mathcal{Q}}
\def\Rscr{\mathcal{R}}
\def\Sscr{\mathcal{S}}
\def\Tscr{\mathcal{T}}
\def\Uscr{\mathcal{U}}
\def\Vscr{\mathcal{V}}
\def\Wscr{\mathcal{W}}
\def\Zscr{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Delta quantities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dd{\Deltait d}
\def\dx{\Deltait x}
\def\dy{\Deltait y}
\def\dz{\Deltait z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computer packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Matlab{\textsc{Matlab}}
\newcommand{\code}[1]{{\small#1}}
\def\KNOSSOS{\code{KNOSSOS}}
\def\MINOS  {\code{MINOS}}
\def\LANCE  {\code{LANCELOT}}
\def\SNOPT  {\code{SNOPT}}
\def\SLQP   {S$\ell_1$QP}
\def\QPSOL  {\code{QPSOL}}
\def\LUSOL  {\code{LUSOL}}
\def\LSSOL  {\code{LSSOL}}
\def\GAMS   {\code{GAMS}}
\def\AMPL   {\code{AMPL}}
\def\COPS   {\code{COPS}}
\def\CUTE   {\code{CUTE}}
\def\CUTEr  {\code{CUTEr}}
\def\ADIC   {\code{ADIC}}
\def\CONOPT {\code{CONOPT}}
\def\NEOS   {\code{NEOS}}
\def\cpp    {C\raisebox{0.1ex}{\hbox{\small++}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Sec{\S}
\def\seq#1{\ensuremath{\{#1\}}}
\newcommand{\e}[1]{e\raisebox{.2ex}{\tiny$#1$}} % scientific not. (e)
\newcommand{\ozguryilmaz}{{\"O}zg{\"u}r Y{\i}lmaz}  % Ozgur Yilmaz's full name!
\newcommand{\ozgur      }{{\"O}zg{\"u}r}            % Ozgur Yilmaz's name!

==> tables/TableTrajectoryStatus.tex <==
\begin{tabular}{rp{5pt}>{\raggedleft\arraybackslash}p{16pt}>{\raggedleft\arraybackslash}p{16pt}p{0pt}>{\raggedleft\arraybackslash}p{16pt}>{\raggedleft\arraybackslash}p{16pt}p{0pt}>{\raggedleft\arraybackslash}p{16pt}>{\raggedleft\arraybackslash}p{16pt}}
&&\multicolumn{8}{c}{\#Successful}\\
\cline{1-1}\cline{3-10}
$k$&&\multicolumn{2}{c}{Backtrack}&&\multicolumn{2}{c}{Local}&&\multicolumn{2}{c}{Global}\\
&&\multicolumn{2}{c}{}&&\multicolumn{2}{c}{trajectory}&&\multicolumn{2}{c}{trajectory}\\
\cline{1-1}\cline{3-4}\cline{6-7}\cline{9-10}
\\[-9pt]
 50&&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\[3pt]
100&&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\[3pt]
150&&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\[3pt]
200&&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  20&  20\\[3pt]
\multicolumn{10}{c}{({\bf{a}}) Tolerance $10^{-4}$}\\[10pt]
 50&&  20&  20&&  19&  20&&  20&  20\\
   &&  20&  20&&  19&  20&&  20&  20\\
   &&  18&  20&&  20&  20&&  19&  20\\[3pt]
100&&  17&  20&&  20&  20&&  20&  20\\
   &&  20&  20&&  20&  20&&  19&  20\\
   &&  19&  20&&  20&  20&&  19&  20\\[3pt]
150&&  17&  20&&  19&  20&&  20&  20\\
   &&  19&  20&&  20&  20&&  20&  20\\
   &&  15&  20&&  19&  20&&  18&  20\\[3pt]
200&&  14&  20&&  18&  20&&  15&  20\\
   &&  14&  20&&  19&  20&&  17&  20\\
   &&  12&  20&&  12&  20&&  11&  20\\[3pt]
\multicolumn{10}{c}{({\bf{b}}) Tolerance $10^{-6}$}\end{tabular}
